Inference-time Stochastic Ranking with Risk Control

Learning to Rank (LTR) methods are vital in online economies, affecting users and item providers. Fairness in LTR models is crucial to allocate exposure proportionally to item relevance. Widely used deterministic LTR models can lead to unfair exposure distribution, especially when items with the same relevance receive slightly different ranking scores. Stochastic LTR models, incorporating the Plackett-Luce (PL) ranking model, address fairness issues but suffer from high training cost. In addition, they cannot provide guarantees on the utility or fairness, which can lead to dramatic degraded utility when optimized for fairness. To overcome these limitations, we propose Inference-time Stochastic Ranking with Risk Control (ISRR), a novel method that performs stochastic ranking at inference time with guanranteed utility or fairness given pretrained scoring functions from deterministic or stochastic LTR models. Comprehensive experimental results on three widely adopted datasets demonstrate that our proposed method achieves utility and fairness comparable to existing stochastic ranking methods with much lower computational cost. In addition, results verify that our method provides finite-sample guarantee on utility and fairness. This advancement represents a significant contribution to the field of stochastic ranking and fair LTR with promising real-world applications.

==> abs.tex <==
 Learning to Rank (LTR) methods are essential for influential applications such as search and recommendation systems, playing a critical role in online economies and impacting not only users but also people behind the items (e.g., sellers and content providers). Therefore, it is crucial to guarantee the fairness in ranking systems such that items are allocated with exposure proportional to their relevance.
 The widely used traditional deterministic ranking systems can result in an unfair distribution of exposure to items, especially when they predict slightly different ranking scores for items sharing the same merit. While the Plackett-Luce (PL) model have been incorporated to stochastic ranking systems to address these fairness issues, they present significant drawbacks such as computational costliness and lack of performance guarantees. To tackle these limitations, we introduce a novel post-hoc model-agnostic method, Fair Learning to Rank with Distribution-free Risk Control (FairLTR-RC). The proposed method can create a stochastic ranking system using any pre-existing scoring function, without requiring expensive training, and can provide guarantees on a specified metric based on distribution-free risk control. Our approach incorporates a novel partially stochastic ranking model, the Thresholded PL (TPL) model, to effectively balance utility and fairness. Experimental results on various benchmark datasets demonstrate that our method significantly enhances fairness in widely-used scoring functions, outperforming state-of-the-art stochastic ranking systems while providing a predefined level of utility. This represents a significant step forward in the field of fair LTR, with potential for broad real-world application.



==> back_up.tex <==
\subsection{Guarantee on Fairness Metric}

Here, we define the score function on ranking lists.
%
Given a PL ranking model $f$ and a query $q$, we have predicted ranking list $P(\hat{Y}|q)=f(q)$.
%
For predicted ranking list $\hat{Y}$, let $s(\hat{Y})$ be its predicted score.
%
$P(\hat{Y}|q)$ is non-decreasing w.r.t. $s(\hat{Y})$.
%
Let $\mathcal{T}_{\lambda}^0$ and $\mathcal{T}_{\lambda}^1$ denote the predicted set of ranking lists given the threshold for guarantee on ranking metric and fairness metric:
\begin{equation}
    \mathcal{T}^0_{\lambda_0}(q) = \{\hat{Y}:s(\hat{Y})\ge \lambda_0\},
    \mathcal{T}^1_{\lambda_1}(q) = \{\hat{Y}:s(\hat{Y})\ge 1-\lambda_1\}
\end{equation}

We consider exposure based fairness metrics, where exposure is determined by the position.
%
Under PL ranking model, the exposure of an item $d$ is written as the expected exposure over the predicted distribution of ranking lists:
\begin{equation}
    \mathcal{E}(d,q) = \sum_{\hat{Y}} P(\hat{Y}|q) \sum_{k=1}^K \theta_k \mathds{1}(\hat{y}_k=d).
\end{equation}
%
\begin{equation}
    \mathcal{R}_{fair}(q) = \sum_{d \in \mathcal{D}_q}\sum_{d'\in \mathcal{D}_q \setminus \{d\}} (\mathcal{E}(d,q)\rho_{d',q} - \mathcal{E}(d',q)\rho_{d,q})^2,
\end{equation}
where $\mathds{1}(\cdot)$ is the indicator function.

The ranking risk $\mathcal{R}_{risk}$ (e.g., negative NDCG) is non-decreasing as we include more ranking lists, in other words, it is non-increasing as $\lambda_0$ increases.

The fairness disparity metric $\mathcal{R}_{fair}$ is non-increasing as we include more ranking lists ($\lambda_1$ increases).
%

We first consider the situation where we need the guarantee on the fairness metric while maximizing the ranking metric, which is similar to widely adopted constrained optimization problem in the literature.
% Our final goal is to have guarantee on both ranking and fairness metrics by taking the intersection of $\mathcal{T}^0_{\lambda_0}(q) \cap \mathcal{T}^1_{\lambda_1}(q)$.
% \begin{equation}
%         P(\mathcal{R}_{rank} > \alpha_{rank}) < \delta_{rank}
% \end{equation}
% %
\begin{equation}
\begin{split}
& \arg \min_{\lambda_1} \; \mathcal{R}_{rank}(\mathcal{S}_{\lambda_1},q)
\\
   &  s.t. \; P(\mathcal{R}_{fair} > \alpha_{fair}) < \delta_{fair},
\end{split}
\end{equation}
where $\mathcal{S}_{\lambda_1}$ is obtained through:
\begin{equation}
    \mathcal{S}_{\lambda_1}(q) = \underset{\mathcal{S}'\subset \mathcal{T}^1_{\lambda_1}}{\arg\min}  \; \mathcal{R}_{rank}(\mathcal{S}',q),
\end{equation}
where $\mathcal{R}(\mathcal{S}',q) = \frac{\sum_{\hat{Y}\in \mathcal{S}'}P(\hat{Y}|q)\mathcal{R}_{rank}(\hat{Y})}{\sum_{\hat{Y}\in \mathcal{S}'}P(\hat{Y}|q)}$ is the expected ranking metric for the set $\mathcal{S}'$ under the PL ranking model.

\subsection{Non-increasing Fairness Disparity Measure}

The expected exposure of item $d$ in query $q$ when only consider ranking lists in $\mathcal{T}^1_{\lambda_1}$ can be written as:
\begin{equation}
    \mathcal{E}(d,q|\mathcal{T}^1_{\lambda_1}) = \frac{\sum_{\hat{Y}\in \mathcal{T}^1_{\lambda_1}} P(\hat{Y}|q) \sum_{k=1}^K \theta_k \mathds{1}(\hat{y}_k=d)}{\sum_{\hat{Y}\in \mathcal{T}^1_{\lambda_1}} P(\hat{Y}|q)}.
\end{equation}
Thus, when $\lambda_1$ increases, we include more ranking lists.
%
Assuming that $ \lambda_1 < \lambda_1'$, we aim to show that:
\begin{equation}
    \mathcal{R}_{fair}(q|\mathcal{T}^1_{\lambda_1}) \ge  \mathcal{R}_{fair}(q|\mathcal{T}^1_{\lambda_1'})
\end{equation}

Consider $(d,d')$, we have:
\begin{equation}
    (\mathcal{E}(d|\lambda_1)\rho_{d'}-\mathcal{E}(d'|\lambda_1)\rho_{d})^2 - (\mathcal{E}(d|\lambda_1')\rho_{d'}-\mathcal{E}(d'|\lambda_1')\rho_{d})^2
\end{equation}


The risk function can be a negative ranking metric.
%
Here, for simplicity, we use ranking metric in the form of:
\begin{equation}
    \mathcal{R}_{risk}(\bm{
    \lambda}) = - \mathds{E}_{\hat{Y}\sim P(\hat{Y}|\bm{\lambda})}[\sum_{k=1}^K \theta_k \rho_d],
\end{equation}
where $P(\hat{Y}|\bm{\lambda})$ is the distribution induced by $\mathcal{T}^1_{\lambda_1},...,\mathcal{T}^k_{\lambda_k}$ and a distribution $P(d|\mathcal{T}^k_{\lambda_k})$ over items in the predicted set for position $k$. Note that by defining a proper $P(d|\mathcal{T}^k_{\lambda_k})$, we can turn any deterministic ranker into a stochastic one, which has guarantee on ranking metric and better item exposure fairness. This allows us to avoid the expensive computational cost of training PL ranking models with policy gradient while enjoy its benefit w.r.t. fairness.
%
$\bm{\lambda}$ is the set of thresholds, each of them is for one of the $K$ positions. $\theta_k$ is the weight of position $k$ and $\rho_d$ is the relevance of item $d$.
%

\subsection{Ranking as A Sequence of Classification Problems}

In~\cite{chen2009ranking}, Chen et al. propose the essential loss, which upper bounds the risk functions corresponding to widely used ranking metrics, e.g., $1-NDCG$ and $1-MAP$.
%
This is based on the fact that ranking can be considered as a sequence of classification problems.
%
The essential loss is a $1/0$ loss:
\begin{equation}
    L_{ess} = \sum_{k=1}^{K}\theta_{k}(1-\prod_{i=k+1}^K \mathds{1}(s_{y^*(k)} > s_{y^*(i)} )),
\end{equation}
where $y^*(k)$ denotes the item index on the $k$-th position in a optimal ranking list $y^* \in \mathcal{Y}^*$. Note that we it is possible to have multiple optimal ranking list for each search session, i.e., $|\mathcal{Y}^*|>1$.
%

In our case, an issue of the essential loss is that it assumes there is only one optimal item for a given position, leading to the term $\mathds{1}(s_{y^*(k)}>s_{y^*(i)})$.
%
For improving item exposure fairness, we relax the essential loss to consider items that are equally well or slightly worse to be .
%
This leads to the following set-valued risk function:
\begin{equation}
       L_{novel} = \sum_{k=1}^{K}\theta_{k}(1-\mathds{1}()),
\end{equation}
where $D_{k}^* = \{d|l_d = 1 \cap y_{1:k-1}\}$

The key is to guarantee the FPR in the top positions.

\subsection{score function}

We define the score of item $d$ at position $k$ to be the expected probability to sample item $d$ at position $k$, given $P(d|\emptyset)$ predicted by a ranker:
\begin{equation}
\scriptsize
s_k(d) =
\begin{cases}
\mathds{E}_{y_{1:k-1}} [P(d|y_{1:k-1})] = \sum_{y_{1:k-1}} P(y_{1:k-1})P(d|y_{1:k-1}) & if \;\; k > 1 \\
P(d|\emptyset) & if \;\;  k=1
\end{cases}
\end{equation}
where $P(d|y_{1:k-1})$ can be obtained from Eq.~\eqref{eq:pl_rank} and $P(y_{1:k-1}) = P(d|y_{1:k-2})P(y_{1:k-2})$ can be computed accordingly.
%
Practically, we can either \begin{itemize}
    \item adopt the reparameterization trick \cite{bruch2020stochastic,oosterhuis2021computationally} to approximate $s_k(d)$ by Monte Carlo with the Gumble noise or
    \item use a heuristic score to replace $p_d$, like a function of the ranking scores (e.g., $\log(s_d)$) as the the score function.
\end{itemize}

==> fig_abstain.tex <==

\begin{figure*}[tbh!]
  \centering
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{./figs/yahoo/HB/cat-query-rmse_scaling_1.0}
    \subcaption{\cat \ on Yahoo, $\lambda$ selected by Hoeffding-Benktus.}
    \label{fig:coverage_cat_yahoo}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/yahoo/HB/lambdaloss_scaling_1.0}
    \caption{NN on Yahoo, $\lambda$ selected by Hoeffding-Benktus.}
    \label{fig:coverage_NN_yahoo}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
\includegraphics[width=\linewidth]{figs/mslr/HB/cat-query-rmse_scaling_1.0.png}
    \caption{\cat \ on MSLR, $\lambda$ selected by Hoeffding-Benktus.}
    \label{fig:coverage_NN_yahoo}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
\includegraphics[width=\linewidth]{figs/mslr/HB/lambdaloss_scaling_1.0.png}
    \caption{NN on MSLR, $\lambda$ selected by Hoeffding-Benktus.}
    \label{fig:coverage_NN_yahoo}
  \end{subfigure}
  \caption{Number of times that FairLTR-RC abstains from selecting the threshold $\lambda$ (y-axis) under various calibration ratio (x-axis) over 50 random data splits with \cat \ and NN. 
  % Results for other datasets, and \lgb \ can be found in Appendix~\ref{sec:detailed_results}.
  % The red (green) vertical line is the desired NDCG@5 level $1-\alpha = 0.9 U^*$, where $U^*$ denotes the NDCG@5 of the deterministic model.
  }
  \label{fig:abstain}
\end{figure*}

==> packages.tex <==
\usepackage{bm}
\usepackage{dsfont}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{multirow}
\usepackage{amsmath}

\usepackage{graphicx}
\usepackage{subcaption}

\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
%%
%% end of the preamble, start of the body of the document source.
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{amsmath}
\usepackage{cleveref}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{thmtools}


==> tab_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|ccccccc|}
\hline
\multicolumn{7}{|c|}{Yahoo}                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|c|}{$f$}                              & \multicolumn{1}{c|}{$\pi$}                 & \multicolumn{1}{c|}{Risk Ctrl}                  & \multicolumn{1}{c|}{1-$\alpha$} & \multicolumn{1}{c|}{NDCG@5}              & \multicolumn{1}{c|}{$R_{sq-fair}$}     & $R_{abs-fair}$    \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{Catboost}}        & \multicolumn{1}{c|}{Det}                   & \multicolumn{1}{c|}{--}                         & \multicolumn{1}{c|}{--}         & \multicolumn{1}{c|}{0.763 $\pm$ 0.003}   & \multicolumn{1}{c|}{1.874 $\pm$ 0.043} & 0.675 $\pm$ 0.007 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{PL}                    & \multicolumn{1}{c|}{--}                         & \multicolumn{1}{c|}{--}         & \multicolumn{1}{c|}{0.648 $\pm$ 0.002}   & \multicolumn{1}{c|}{0.975 $\pm$ 0.043} & 0.487 $\pm$ 0.008 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\multirow{3}{*}{ours}} & \multicolumn{1}{c|}{\multirow{3}{*}{Greedy-HB}} & \multicolumn{1}{c|}{0.74}       & \multicolumn{1}{c|}{0.758 $\pm$ 0.005}   & \multicolumn{1}{c|}{1.698 $\pm$ 0.071} & 0.635 $\pm$ 0.014 \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{0.732}      & \multicolumn{1}{c|}{0.751 $\pm$ 0.005}   & \multicolumn{1}{c|}{1.576 $\pm$ 0.057} & 0.61 $\pm$ 0.011  \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{0.725}      & \multicolumn{1}{c|}{0.746   $\pm$ 0.004} & \multicolumn{1}{c|}{1.5 $\pm$ 0.051}   & 0.596 $\pm$ 0.009 \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{Lightgbm}}        & \multicolumn{1}{c|}{Det}                   & \multicolumn{1}{c|}{--}                         & \multicolumn{1}{c|}{--}         & \multicolumn{1}{c|}{0.763 $\pm$ 0.003}   & \multicolumn{1}{c|}{1.899 $\pm$ 0.048} & 0.676 $\pm$ 0.008 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{PL}                    & \multicolumn{1}{c|}{--}                         & \multicolumn{1}{c|}{--}         & \multicolumn{1}{c|}{0.645 $\pm$ 0.002}   & \multicolumn{1}{c|}{0.984 $\pm$ 0.043} & 0.485 $\pm$ 0.008 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\multirow{3}{*}{ours}} & \multicolumn{1}{c|}{\multirow{3}{*}{Greedy-HB}} & \multicolumn{1}{c|}{0.74}       & \multicolumn{1}{c|}{0.758 $\pm$ 0.005}   & \multicolumn{1}{c|}{1.725 $\pm$ 0.07}  & 0.636 $\pm$ 0.014 \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{0.732}      & \multicolumn{1}{c|}{0.752 $\pm$ 0.005}   & \multicolumn{1}{c|}{1.615 $\pm$ 0.056} & 0.613 $\pm$ 0.01  \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{0.725}      & \multicolumn{1}{c|}{0.746 $\pm$ 0.005}   & \multicolumn{1}{c|}{1.541 $\pm$ 0.053} & 0.598 $\pm$ 0.01  \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{NN}} & \multicolumn{1}{c|}{Det}                   & \multicolumn{1}{c|}{--}                         & \multicolumn{1}{c|}{--}         & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                  &                   \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{PL}                    & \multicolumn{1}{c|}{--}                         & \multicolumn{1}{c|}{--}         & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                  &                   \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\multirow{3}{*}{ours}} & \multicolumn{1}{c|}{\multirow{3}{*}{Greedy-HB}} & \multicolumn{1}{c|}{0.74}       & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                  &                   \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{0.732}      & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                  &                   \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{0.725}      & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                  &                   \\ \hline
\end{tabular}
\end{table}
